Observational signatures of outbursting protostars -- II: Exploring a wide range of eruptive protostars

Young stars exhibit variability due to changes in the gas accretion rate onto them, an effect that should be quite significant in the early stages of their formation. As protostars are embedded within their natal cloud, this variability may only be inferred through long wavelength observations. We perform radiative transfer simulations of young stellar objects (YSOs) formed in hydrodynamical simulations, varying the structure and luminosity properties in order to estimate the long-wavelength, sub-mm and mm, variations of their flux. We find that the flux increase due to an outburst event depends on the protostellar structure and is more prominent at sub-mm wavelengths than at mm wavelengths; e.g. a factor of 40 increase in the luminosity of the young protostar leads to a flux increase of a factor of 10 at 250 micron but only a factor of 2.5 at 1.3 mm. We find that the interstellar radiation field dilutes the flux increase but that this effect may be avoided if resolution permits the monitoring of the inner regions of a YSO, where the heating is primarily due to protostellar radiation. We also confirm that the bolometric temperature and luminosity of outbursting protostars may result in an incorrect classification of their evolutionary stage.

==> README <==
% readme.txt
%
% MNRAS journal LaTeX package
% v3.0 for LaTeX 2e
%
%
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%   http://www.latex-project.org/lppl.txt
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
%
% This work has the LPPL maintenance status `author-maintained'.
% 
% The Current Maintainer of this work is: Royal Astronomical Society,
% MNRAS Editorial Office, who can be contacted on mn@ras.org.uk
%
% This work consists of all the files listed in readme.txt
%
%
% Last updated 22 May 2015
%
% Copyright (C) Royal Astronomical Society 2015, Blackwell Science 2001,
% Cambridge University Press 1994
%
% See each file for a detailed author list and change log.
%
% This package consists of the following files:

readme.txt          This file

mnras.cls           MNRAS LaTeX document class
mnras.bst           MNRAS BibTeX style

mnras_guide.tex     User guide, LaTeX format
mnras_guide.pdf     User guide, PDF format
mnras_template.tex  A simple template paper

example.eps         An example image used in the guide
example.png         An example image used in the guide
example.ps          An example image used in the guide

legacy\legacy.txt   Description of the legacy releases
legacy\mn2e.cls     v2.2 of mn2e.cls (deprecated)
legacy\mn2e.bst     v1.1b of mn2e.bst (deprecated)


% Disclaimer:
%
% This LaTeX package is provided free to the community in the hope that it
% assists them in preparing papers for the journal Monthly Notices of the
% Royal Astronomical Society.
% The files are provided 'as-is' with no guarantee of their suitability,
% freedom from errors or omissions, or compatibility with any software.
% The Royal Astronomical Society cannot provide user support for this package,
% LaTeX, or for any other software.
% Authors are free to use other styles or programmes if they wish.
% Please see the journal instructions to authors for guidance.
% This disclaimer is in addition to the No Warranty section of the licence,
% at the link given above.
